Trident: Interference Avoidance in Multi-reader Backscatter Network via Frequency-space Division

Backscatter is a key technology for battery-free sensing in industrial IoT applications. To fully cover numerous tags in the deployment area, one often needs to deploy multiple readers, each of which communicates with tags within its communication range. However, the actual backscattered signals from a tag are likely to reach a reader outside its communication range and cause interference. Conventional TDMA or CSMA based approaches for interference avoidance separate readers' media access in time, leading to limited network throughput. In this paper, we propose TRIDENT, a novel backscatter design that enables interference avoidance via frequency-space division. By incorporating a tunable bandpass filter and multiple terminal loads, a TRIDENT tag can detect its channel condition and adaptively adjust the frequency and the power of its backscattered signals. We further propose a frequency assignment algorithm for the readers. With these designs, all the readers in the network can operate concurrently without being interfered. We implement TRIDENT and evaluate its performance under various settings. The results demonstrate that TRIDENT enhances the network throughput by 3.18x, compared to the TDMA-based scheme.

==> src/3_reader_frequency_assignment.tex <==
\section{Reader Frequency Assignment}

% \SystemName工作的前提条件是Backscatter network中相邻的Reader使用不同的工作频率。而在本章节中，我们提出了一个算法来指配Reader的工作频率，让相同频率的Reader相互远离以避免同频干扰。此外，我们在在两种不同的多Reader部署环境下使用该算法进行了simulation，验证其可以在较短时间内给出同频干扰较少的Reader频率指配方法。

\SystemName tags are required to operate in a backscatter network where the adjacent readers work at different bands. In this section, we propose an algorithm to assign the readers' working frequency band. This algorithm separates the same-band readers to avoid interference. Besides, We conducted simulations in two multi-reader deployment scenarios to validate this algorithm.

% 一种理想的情况是如LTE的基站那样使用hexagonal grid modeled deployment，in which仅需要三个不同的频段就可以实现相邻cell之间的干扰避免，如图Fig. \ref{}所示。然而在实际的IIoT场景中，Reader的部署位置往往受到多种因素的制约，将Reader按照hexagonal grid部署并不现实。

In an ideal scenario, we can employ a hexagonal grid deployment model similar to LTE base stations. This requires only three different frequency bands to avoid interference between adjacent cells, as illustrated in Fig. \ref{}. However, in real IIoT environments, reader deployment locations are often constrained by various factors, making it impractical to deploy readers in a hexagonal grid pattern.

% ！！！
% 这里第一步就应该先说明白：解的存在性的问题。举例子、给出充分条件之类的方法，说明完全不干扰的解普遍的不存在，然后再来讨论怎么量化它的好坏呢？使用干扰强度来量化好坏，干扰的减少是我们的目标。
% ！！！

% 为了在Reader部署位置受限的情况下避免同频干扰，我们需要小心地分配每个Reader的频率。然而，这是一个NP难问题。每个Reader的工作频段可以在\SystemName tag支持的三个频段中任意选择，对于数十个Reader的场景下，遍历所有的解会带来O(3^n)的复杂度，which is unacceptable。为此，我们将上述问题建模为一个优化问题。考虑到Reader的频率指配是一个离散变量的优化问题，我们使用了启发式的遗传算法求解。

To avoid co-frequency interference in scenarios where reader deployment is constrained, we need to assign frequencies to each reader carefully. However, this poses an NP-hard problem. Each reader's operating frequency band can be chosen from the three bands supported by the \SystemName tag. For scenarios involving dozens of readers, traversing through all possible solutions results in a complexity of $O(3^n)$, which is unacceptable. To tackle this, we model this problem as an optimization problem. Considering that frequency assignment for readers is an optimization problem with multiple discrete variables, we utilized a heuristic genetic algorithm to solve it.

% 该算法以每个Reader分配的频率作为优化的对象，将最小化同频干扰信号的能量作为优化的目标。考虑到电磁波在空间中的衰减和距离的平方成正比，我们将同频干扰的能量定义为某Reader到其他所有同频Reader的距离的平方的倒数的求和。具体算法如Alg.\ref{alg:frequency-assign}所示。

The algorithm optimizes the frequency assigned to each reader, aiming to minimize the energy of co-frequency interference signals. Considering the proportional relationship between the attenuation of RF signals in space and the square of the distance, we define the energy of co-channel interference as the sum of the reciprocal of the distance squires between a specific reader and all other co-frequency readers. The detailed algorithm is depicted in Alg. \ref{alg:frequency-assign}.

\begin{algorithm}[t]
    \SetKwRepeat{Do}{do}{while}
    \SetAlgoLined
    \caption{Reader\ Frequency\ Assignment\ with\ Genetic\ Algorithm}
    \label{alg:frequency-assign}
    \KwIn{$P_i=[x_i, y_i]$: 2D location of readers}
    \KwOut{$F$: Reader frequency assignment strategy}
    \BlankLine
    Randomly initialize population $G_0=[F_0, F_1, \cdots, F_{M-1}]$\;
    $cnt \gets 0$\;
    \Do{$cnt < C$}{
        \For{$F_{i} \text{ in } G_{cnt}$}{
            \ForEach{Reader $R_j$}{
                Find same-band readers $R_{jk}$\;
                $D_{jk} \gets \sqrt{(x_i-x_j)^2+(y_i-y_j)^2}$\;
                $E_j \gets \sum_{k}1/D_{jk}^2$\;
                $Error_i \gets \text{mean}(E_j) + \text{median}(E_j, 0.5)$\;
            }
        }
        $G_{cnt} \gets \text{top 10\% individuals of } G_{cnt}$,
        ascending sorted by $Error_i$\;
        $G_{cnt+1} \gets \text{mate, mutate, expansion }(G_{cnt})$\;
        $cnt \gets cnt + 1$\;
    }
    $F \gets F_{i} \text{ in } G_C \text{ with minimum } Error_i$\;
\end{algorithm}

% 算法的输入为$N$个Reader的位置，输出为优化后的Reader频率指配策略$F$。The processing unfolds as the following steps:（使用Reader的位置作为输入是并不合理的！应该改成实际测量的结果）

This algorithm takes the location of $N$ readers as the input and outputs the optimized frequency assignment strategy $F$. The processing unfolds as the following steps:

% 我们初始化$M$种工作频率指配$F_{i}$作为个体，where $M$是种群数量 and $i \in [0, M-1]$。

% 对于种群内每个分配方法$F_{i}$，我们计算在该分配方法下每个Reader收到的干扰能量$E_{j}$，where $j \in [0, N-1]$，并且使用$E_{j}$中最大值与$E_{j}$的中位数的和作为error。这样选择的目的是希望该优化能同时兼顾局部和全局。

% 选取出error最小10%的个体，利用经典的遗传算法执行交换基因、种群扩充、变异等步骤，并进行下一轮的评估，直到迭代次数达到预设限制。

\begin{enumerate}
    \item We initialize $M$ sets of frequency assignment as the individuals in population $G_0$. Each frequency assignment is represented by $F_i$, where $i \in [0, M-1]$ (Line 1).

    \item For each assignment method $F_{i}$ within the population, we calculate the interference energy $E_{j}$ received by each reader under this assignment method, where $j \in [0, N-1]$. We use the sum of the maximum value in $E_{j}$ and the median of $E_{j}$ as the error. This selection aims to ensure that the optimization considers both local and global aspects simultaneously (Line 4-11).

    \item We select the top 10\% individuals with the lowest error and employ classic mating, mutation, and population expansion methods to generate the next generation. Then we proceed with the next round of evaluation until the iteration count reaches the preset limit (Line 12-14).

    \item Finally we output the individual with minimum error in population $G_{C}$ as the optimized reader frequency assignment strategy (Line 16).
\end{enumerate}

% 为了验证上述算法的有效性，我们构建了两种Reader的部署环境，每个环境中有20个Reader。我们使用该算法为这些Reader分配频率，通过...评估频率分配的合理性。我们另外使用随机生成100k个策略取最优的方法作为Baseline。

% Simulation的场景与结果如Fig.\ref{}所示。

==> src/7_discussion.tex <==
\section{Discussion}
\label{title:discussion}

\subsection{Frequency Band}

Due to the broad bandwidth of the tunable bandpass filters, we currently set the operating frequency options to 700MHz, 800MHz, and 900MHz. However, not all three frequency bands fall within the ISM frequency range, which does not meet the requirements for practical deployment. If we utilize filters with narrower bandwidth, the operating frequency bands of the \SystemName can be set into the narrow ISM band. The Surface Acoustic Wave (SAW) filter is a new type of filter that can provide ultra-narrow bandwidth as low as 2\% in 915MHz ISM frequency band\cite{datasheetmuratasaw}. In the downlink design for backscatter communication, some works have leveraged the excellent performance of SAW filters \cite{guo2022saiyan, li2022passive}. By incorporating a set of such filters with different center frequencies in \SystemName tags, we can meet the requirements for the operating frequency bands that ensure widespread application in real-world scenarios.

\addsec
\subsection{Reader Transmission Power Adjustment}
% The working frequencies and deployment positions of readers in \SystemName network need to be carefully configured. Inspired by cellular networks \cite{novlan2011analytical}, we can utilize a hexagonal frequency reuse network deployment: readers located within adjacent hexagons operate on different frequency bands, while the same frequency bands are reused by readers in non-adjacent hexagons, as depicted in Fig. \ref{fig:frequency-reuse-network}. Such a layout simultaneously satisfies the requirements of frequency and spatial division, making it a potential reader deployment approach for \SystemName network.

% 在一些部署环境中，当一个Reader周围有过多的tag时，这个tag都会选择与该reader通信，从而造成严重的tag to tag碰撞与干扰。除了使用一些经典的interference avoidance或者parallel decoding方案以外，我们还可以考虑利用多reader的优势解决该问题。例如我们可以参考\cite{}中的方案，让reader根据自身通信负载动态地降低发射功率，让一些tag选择其他的reader，避免过多tag在某个reader处发生碰撞和拥塞。

In some deployment scenarios, excessive tags surrounding a reader tend to communicate with it, leading to substantial tag-to-tag collisions and interference. Apart from employing traditional interference avoidance or parallel decoding methods\cite{jin2017fliptracer, hessar2019netscatter}, leveraging multiple readers could address this issue. For instance, as proposed in \cite{cha2007adaptive}, we can dynamically adjust the transmission power based on the reader's load, encouraging some tags to choose alternative readers. This might mitigate the risk of excessive tag collisions and congestion at a single reader.

\color{black}
% \subsection{Tag-tag Interference}

%For example, Saiyan \cite{} utilized the extremely narrow transition band of SAW filters to convert frequency-modulated LoRa signals into amplitude-modulated ones. Passive DSSS \cite{} utilized SAW filters to divide the 915MHz ISM frequency band into two channels, enabling frequency division multiplexing transmission of DSSS signals and spreading codes.

% This would allow legal application and deployment for \SystemName.

% \subsection{Tag-tag Interference}

% In \SystemName, the main focus is on addressing the interference caused by activated tags to other readers in a multi-reader environment. In practical deployments, a single reader simultaneously excites multiple tags, leading to interference between their backscatter signals. This interference makes the reader disable to decode the information from any tag. Researchers call this interference as tag-tag interference. As the number of tags activated by a reader increases, the tag-tag interference becomes more severe, significantly limiting the overall system throughput. It is crucial to address the issue of tag-tag interference when employing \SystemName in real deployments.

% 由于tag-tag interference

==> src/deployment_architecture.tex <==
\section{Deployment Architecture}
\label{title:deployment-architecture}

We propose a reader deployment architecture that could meet the requirements of \SystemName. As shown in Fig. \ref{fig:deployment-architecture}, readers are deployed in a hexagonal grid pattern, with the distance between any two readers being less than twice the excitation distance of the reader in the deployment architecture in order to achieve reliable coverage of the target area. In this deployment architecture, we assign three frequency bands to all readers, which are sufficient to ensure adjacent readers operate on different bands in the hexagonal grid, and avoid interference based on frequency division between neighboring readers and tags.

For readers operating on the same frequency band, we deploy them as far apart as possible from each other in the hexagonal grid. Thus, a reader is unlikely to be interfered by a tag being excited by another distant reader operating at the same frequency. This deployment strategy enables interference avoidance between same-frequency readers based on space division.

Deploying the reader in this manner is not enough to achieve interference avoidance. In the next section, we will introduce backscatter tags specifically designed for \nameofdesign.

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{src/img/network_architecture.pdf}
    \caption{The deployment architecture of placing readers in a hexagonal grid pattern.}
    \label{fig:deployment-architecture}
\end{figure}
